Feminist Interaction Techniques: Deterring Non-Consensual Screenshots with Interaction Techniques

Non-consensual Intimate Media (NCIM) refers to the distribution of sexual or intimate content without consent. NCIM is common and causes significant emotional, financial, and reputational harm. We developed Hands-Off, an interaction technique for messaging applications that deters non-consensual screenshots. Hands-Off requires recipients to perform a hand gesture in the air, above the device, to unlock media -- which makes simultaneous screenshotting difficult. A lab study shows that Hands-Off gestures are easy to perform and reduce non-consensual screenshots by 67 percent. We conclude by generalizing this approach and introduce the idea of Feminist Interaction Techniques (FIT), interaction techniques that encode feminist values and speak to societal problems, and reflect on FIT's opportunities and limitations.

==> 03_fit.tex <==
\section{FIT: Feminist Interaction Techniques} \label{fit}

This paper introduces the concept of \textit{Feminist Interaction Techniques (FIT)}--- interaction techniques that embody feminist values and speak to societal problems. Figure \ref{fig:fit} presents a high-level illustration of the important interplay between \textit{values, problem spaces,} and \textit{interaction techniques} in FIT. FIT aims to translate feminism's values---and its goal of a more just and equitable society through them---into lower-level, technical HCI concepts. FIT best applies to the social aspects of computing, where feminist values can speak to power structures between people and social groups in society.

While some subdomains of computing (e.g. the field of Social Computing \cite{steinhardt2015feminism}) have been receptive to the idea of feminism-inspired designs, systems built with such values are few and far between. Part of the issue is the inherent difficulty of mapping high-level concepts to concrete system interactions. FIT aims to bridge the gap between what values systems should have and how they can be built into interactive technologies, and attempts to be an answer to calls to make feminism concrete in systems~\cite{bardzell_feminist_2010}.

\textbf{Values.} Feminism is a multi-faceted movement and discipline that has evolved through different waves and phases (see a review within the computing context in~\cite{bardzell_feminist_2010}). Feminism, like any set of values or principles, has flaws and limitations (e.g. early feminism prioritized gender while overlooking race, a pattern that was also observed with social technologies \cite{steele2021digital}). However, many of its core values are durable, including consent, boundaries, equity, bodily autonomy, economic justice, and intersectionality. While outside the scope of this paper to exhaustively list values, FIT can leverage any feminist value to create new interaction techniques.

\textbf{Problem spaces.} FIT is a response to voices from scholars to develop novel interaction techniques in social computing systems. Digital safety, and other problem spaces with gendered harms, are natural fits for FIT; however, FIT is not limited to these contexts. There has been much demand for systems and mechanisms that make online interactions safer, more effective, and more inclusive. Figure \ref{fig:fit} shows existing and growing areas that require innovation and tooling in user interfaces and interaction techniques. This includes, but is not limited to, preventing the creation and dissemination of NCIM~\cite{citron2014criminalizing,citron2018sexual, citron2022fight, franks_drafting_2014, geeng2020usable, powell_image-based_2019, mcglynn_its_2021, freed_digital_2017, qin2024did}, protecting our data bodies~\cite{lee_building_2017}, reducing acts of intimate partner violence~\cite{tseng2020tools, zou2021role, freed2018stalker, freed_digital_2017}, preventing doxing~\cite{im_yes_2021}, and other forms of online harms. 

\textbf{Interaction techniques.} Interaction techniques mediate and---in some cases---dictate how, when, and why social computing systems are used. It is possible to think of many different vectors for applying FIT to common social interaction paradigms. For example, how would FIT approach the context of meeting someone's VR avatar? How would FIT approach encountering locations and spaces in AR, given that the history of many locations and spaces are contested (e.g., Indigenous lands)? How might FIT deal with consent in deepfakes? How to do this in different domains remains an open question---and an opportunity for technical HCI research.

\textbf{Opportunities and limitations.} It is important to interrogate the limits of FIT---and any technical approach---in important societal problems. FIT cannot solve gender-based violence. No technology can. Problems like NCIM are technologically-mediated, but the social and societal contexts in which they exist have been around for millennia. The oppression of women and gender minorities, how the law treats these harms, how society treats survivor-victims, etc., are problems that technology cannot single-handedly ``fix.'' For computing communities with techno-solutionist norms, it is important to note that no technology---no matter how clever and well-intentioned---will completely solve complex societal problems. 

At the same time, the computing community has a role to play and a responsibility to bear. Problems like NCIM would not exist without decades of computing work that put cameras and mobile devices into nearly everyone's hands, with few safeguards on their use. Paradigms like FIT, while not solutions, can be steps forward.

==> 08_conclusion.tex <==
\section{Conclusion}


This work bridges technology values with system interactions to focus on consent in online messaging. We implement feminist principles into \sys, introducing a gesture-based approach to reduce screenshots. Evaluation results demonstrate its effectiveness in both deterring unwanted screenshots and furthering user reflection about consent. FIT contributes to a more values-aware approach to building social systems.
